Non-functional Requirements for Machine Learning: Understanding Current Use and Challenges in Industry

Machine Learning (ML) is an application of Artificial Intelligence (AI) that uses big data to produce complex predictions and decision-making systems, which would be challenging to obtain otherwise. To ensure the success of ML-enabled systems, it is essential to be aware of certain qualities of ML solutions (performance, transparency, fairness), known from a Requirement Engineering (RE) perspective as non-functional requirements (NFRs). However, when systems involve ML, NFRs for traditional software may not apply in the same ways; some NFRs may become more prominent or less important; NFRs may be defined over the ML model, data, or the entire system; and NFRs for ML may be measured differently. In this work, we aim to understand the state-of-the-art and challenges of dealing with NFRs for ML in industry. We interviewed ten engineering practitioners working with NFRs and ML. We find examples of (1) the identification and measurement of NFRs for ML, (2) identification of more and less important NFRs for ML, and (3) the challenges associated with NFRs and ML in the industry. This knowledge paints a picture of how ML-related NFRs are treated in practice and helps to guide future RE for ML efforts.

==> todo.tex <==

%\item[\done] Frame the problem

\begin{itemize}
  \item Introduction.
  \begin{todolist}
  \item Address remaining comments (Habib)
  \item [\done] Add more NFR related work (Jennifer)
  \item more about related work (Habib)
  \item [\done] write outline of the rest of the paper (Habib)
  \end{todolist}
  \item Related Work
  \begin{todolist}
  \item [\done]add more to the NFR section (Jennifer) (done, but not well)
  \item [\done]work on the RE for AI section (Habib).  More description on paper.  \item [\done] search for more papers (Jennifer)
  \item [\done] SE for AI need more papers (Jennifer)
  \end{todolist}
  \item RQs
  \item Methodology
  \begin{todolist}
  \item [\done]read guidelines (not by Friday) (Habib)
  \item [\done] go through changes (Jennifer)
  \item [\done] improve qualitative coding section (Habib)
  \item [\done]move text from thematic coding section to later sections (Habib)
  \item [\done]give code names special font \textsf{code} (Habib)
  \item Table II should be updated to remove explanation of codes.  (Habib)
  \end{todolist}
  \item Results
  \begin{todolist}
  \item [\done] better explain codes (Habib)
  \item [\done]add countries to demographics (Habib)
  \item  [\done]make all figures PDF (Habib)
  \item [\done]merge table IV into text (Habib)
  \item [\done]need more results for RQ1.4 (Habib)
  \item [\done]Table VI remove and integrate quotes
  \item [\done]Table VIII remove (Habib)
  \item remove Table II?  Only mention some of the sub-codes and the number of codes.  
  \item [\done]reorder NFrs results in Fig. 2
  \item [\done]increase font size of figures (Habib)
  \item [\done]add counts to leaves for challenges (Habib)
  \item [\done]Table IV and V, remove and integrate into text (Habib)
  \item many quotes are hard to read because the grammar is not correct. In some cases we should go back to the recordings.   
  \item Redraw 3 challenges figures to be smaller, bigger text (Habib)
  \end{todolist}
  \item Discussion
  \begin{todolist}
  \item compare to related work (Habib) 
  \item [\done]go through discussion (Jennifer)
  \end{todolist}
 \item threats to validity 
    \begin{todolist}
    \item [\done]write (Jennifer)
  \end{todolist}
  \item Conclusions
    \begin{todolist}
    \item [\done]go through  (Jennifer)
  \end{todolist}
  \item  Other
  \begin{todolist}
    \item share with interviewees their transcript, ask if it can be public, and then share a draft of this paper, ask not to distribute. 
  \end{todolist}
\end{itemize}
